Natural operations on the Hochschild complex of commutative Frobenius algebras via the complex of looped diagrams

We define a dg-category of looped diagrams which we use to construct operations on the Hochschild complex of commutative Frobenius dg-algebras. We show that we recover the operations known for symmetric Frobenius dg-algebras constructed using Sullivan chord diagrams as well as all formal operations for commutative algebras (including Loday's lambda operations) and prove that there is a chain level version of a suspended Cactus operad inside the complex of looped diagrams. This recovers the suspended BV algebra structure on the Hochschild homology of commutative Frobenius algebras defined by Abbaspour and proves that it comes from an action on the Hochschild chains.

==> pic_multicomp1.tex <==

%\definecolor{cff0000}{RGB}{255,0,0}
%\definecolor{c00ff00}{RGB}{0,255,0}
%
%
%\begin{tikzpicture}[y=0.80pt, x=0.8pt,yscale=-1, inner sep=0pt, outer sep=0pt]
\begin{scope}[scale=1.1]
\path[cm={{0.21586,0.0,0.0,0.21682,(112.09364,225.7964)}},draw=black,line
  cap=butt,miter limit=10.00,line width=1pt]
  (-210.0000,-792.6378)arc(0.000:180.000:35.000)arc(-180.000:0.000:35.000) --
  cycle;\path[draw=black,fill=black,line cap=butt,miter limit=10.00,line
  width=1pt,rounded corners=0.0000cm] (57.0459,36.1348) rectangle
  (62.0459,46.1348);\path[draw=black,line join=miter,line cap=butt,line width=1pt]
  (59.5227,35.5251) .. controls (59.3997,27.3835) and (64.8426,19.3712) ..
  (71.2137,17.7798) .. controls (115.7826,6.6473) and (112.3514,61.5789) ..
  (97.5185,72.2683) .. controls (82.6077,83.0139) and (59.8940,77.3281) ..
  (58.6876,61.4124);\path[draw=cff0000,dash pattern=on 3.20pt off 0.80pt,line join=miter,line
  cap=butt,miter limit=4.00,line width=1pt] (62.9950,43.8514) .. controls
  (60.1298,33.4667) and (68.0912,19.9581) .. (76.1664,19.8597) .. controls
  (116.4694,19.3683) and (104.4788,64.1161) .. (95.1664,69.8663) .. controls
  (82.6180,77.6147) and (67.0928,74.0390) .. (62.9950,63.0277);\path[draw=black,line join=miter,line cap=butt,line width=1pt]
  (102.7377,27.1744) -- (92.3410,36.4500);\path[fill=cff0000] (90,48.362183) node[above right] (text6728) {\textcolor{cff0000}2};\path[draw=cff0000,line join=miter,line cap=butt,line width=1pt]
  (62.9838,44.5053) .. controls (74.9096,45.7788) and (73.7274,61.8492) ..
  (63.1631,63.0277);\path[draw=cff0000,line join=miter,line cap=butt,line width=1pt]
  (68.3102,53.6001) -- (70.3948,58.0297) -- (74.9092,55.4460);\path[draw=cff0000,line join=miter,line cap=butt,line width=1pt]
  (92.7466,65.8077) -- (99.1038,65.7653) -- (98.3504,70.7851);\path[draw=cff0000,line join=miter,line cap=butt,line width=1pt]
  (85.8569,17.7532) -- (79.7005,20.0826) -- (84.0266,24.7416) --
  (84.1930,24.5752);\path[cm={{0.0,-0.21586,0.21682,0.0,(350.4898,-2.36941)}},draw=black,line
  cap=butt,miter limit=10.00,line width=1pt]
  (-210.0000,-792.6378)arc(0.000:180.000:35.000)arc(-180.000:0.000:35.000) --
  cycle;\path[draw=black,line join=miter,line cap=butt,line width=1pt]
  (160.0000,50.3622) -- (108.0000,50.3622);\path[cm={{1.1577,0.0,0.0,1.19134,(-39.45129,-17.76619)}},draw=c00ff00,opacity=0.990,line
  cap=butt,miter limit=4.00,line width=1pt]
  (198.2487,57.5052)arc(0.000:180.000:9.624370 and
  9.143)arc(-180.000:0.000:9.624370 and 9.143) -- cycle;\path[cm={{0.0,-1.0,1.0,0.0,(0.0,0.0)}},draw=black,fill=black,line
  cap=butt,miter limit=10.00,line width=1pt,rounded corners=0.0000cm]
  (-52.6784,160.8282) rectangle (-47.6784,170.8282);\path[draw=black,line join=miter,line cap=butt,line width=1pt]
  (178.0000,42.3622) -- (178.0000,29.3622);\path[fill=black] (181.42407,30.292864) node[above right] (text3945) {\textcolor{c00ff00}1};\path[draw=c00ff00,line join=miter,line cap=butt,line width=1pt]
  (186.4267,47.8972) -- (189.8973,51.7795) -- (192.8973,47.7795);\path[draw=c00ff00,line join=miter,line cap=butt,line width=1pt]
  (172.2867,62.6105) -- (170.2867,57.6105) -- (176.2867,56.6105);
  
  \end{scope}
\path[fill=black] (59,64) node[above right] {$v_1$};
\path[fill=black] (190,61) node[above right] {$v_2$};

